Disentangling Controllable Object through Video Prediction Improves Visual Reinforcement Learning

In many vision-based reinforcement learning (RL) problems, the agent controls a movable object in its visual field, e.g., the player's avatar in video games and the robotic arm in visual grasping and manipulation. Leveraging action-conditioned video prediction, we propose an end-to-end learning framework to disentangle the controllable object from the observation signal. The disentangled representation is shown to be useful for RL as additional observation channels to the agent. Experiments on a set of Atari games with the popular Double DQN algorithm demonstrate improved sample efficiency and game performance (from 222.8% to 261.4% measured in normalized game scores, with prediction bonus reward).

==> trash.tex <==
\subsection{Recap on Deep Q-Learning}

Q-Learning is a reinforcement learning algorithm for finding an optimal %decision making 
policy of a Markov decision process (MDP) %, in which an agent interacts with the environment by taking an action at each discrete time step 
\cite{sutton1998reinforcement}. Specifically, consider an agent operating over discrete time $ t \in {1,\ldots, T} $. At time $t$, the agent receives an observation $o_t$ of the environment state $s_t$, %updates the state $s_t$, 
takes an action $a_t \in A$ in response, and receives an immediate numerical reward $r_t$ from the environment. In the Atari domain, $o_t$ is just the image frame, $a_t$ is the game action that the agent chooses, $r_t$ is the game score changes produced by the game simulator, and $s_t$ is conventionally defined as the stacked $k_q$ ($k_q=4$ in our experiments) frames $(o_{t-k_q+1},\ldots,o_t)$.

The cumulative discounted reward starting from time $t$ is defined as $ R_t = \sum_{\tau =t}^{\infty} \gamma^{\tau-t} r_\tau $ ($\gamma \in [0,1]$ is the discount factor). A policy $\pi$ is optimal in the sense that the expected cumulative reward following policy $\pi$ is maximized.
Q-Learning concerns about learning an action-value function, usually referred to as the Q function of policy $pi$ when actions are taken according to $\pi$:
\begin{equation}
	Q^\pi (s,a) = \mathbb{E} [R_t | s_t=s, a_t=a; \pi]
\end{equation}
Under deterministic policy $\pi(s)=\arg \max_{a'\in A}  Q^\pi (s,a')$, it can be shown that the optimal Q function, denoted by $Q^*$ should satisfy the Bellman equation:
\begin{equation}
	Q^* (s,a) = \mathbb{E}_{s'} \left[r + \gamma \max_{a'\in A} Q^*(s',a') | s, a \right]
\end{equation}
where $s'$ is distributed according to state transition dynamic when action $a$ is taken at state $s$.

Deep Q-Learning involves using a deep neural network $Q(s,a;\theta)$ parameterized by $\theta$ as function approximator to Q function. It's typically a CNN on vision-based RL problems such as Atari games. The introduction of CNN enables automatic learning of visual features for control, alleviating the necessity of hand-crafting features. In order to train the Q network, a sequence of loss functions $L_i$ are minimized iteratively as follows:
\begin{align}
	\label{eq_dqn}
	&L_i(\theta_i) = \mathbb{E} \left[ (y_i - Q(s,a;\theta_i) )^2 \right] \\
	\text{with}\quad &y_i = r + \gamma \max_{a'} Q(s',a';\theta_i^-)
\end{align}
where $\theta_i^-$ represents the parameter of a target Q network which is updated periodically to stabilize the training.

In this paper, we adopt the improved Double DQN (DDQN) agent proposed in \cite{DBLP:conf/aaai/HasseltGS16}, which mitigates the over-estimation problem of the original DQN by doing evaluation and argmax with separate Q networks as in Eq~\ref{eq_ddqn}.
\begin{equation}
	\label{eq_ddqn}
	y_i = r + \gamma Q(s', \arg\max_{a'} Q(s',a';\theta^-); \theta_i)
\end{equation}



\begin{algorithm}[ht]
\small
	\SetAlgoLined
	\KwResult{Parameters of the Q function and the prediction net }
	initialize replay buffer $H$, and observe $o_0$\;
	\For{$t = 1 \to T$}{
		choose action $a_t$, and observe $o_{t+1}, r_t$\;
		compute bonus with $o_{t-k+1:t+1}, a_t$ to get $r_{t,aug}$\;
		store $(o_t,a_t,r_{t,aug},o_t+1)$ to replay buffer $H$\;
		%\equiv
		\If{ $t\mod k_p = 0$}{
			sample minibatch $B'$ of transitions from $H$\;
			train prediction model with $B'$ and loss \ref{eq_loss_all}\;
		}
		\If{ $t\mod k_q = 0$}{
			sample another minibatch $B$ from $H$\;
			pass $B$ to prediction model to get the masks\;
			train $Q(;\theta)$ with both $B$ and masked $B$ as input images\;
		}
	}
	\caption{Double DQN + Prediction and Bonus}
	\label{algo_1}
\end{algorithm}


\begin{table}[h]
\small
    \centering
    \caption{Hyper-parameter settings}
    \begin{tabular}{cc}
        \toprule
        Parameter & Value \\
        \midrule
        Q Learning rate & 1e-4 anneal to 0 \\
        Prediction model lr & 1e-3 \\
        T & 1e7 / 4 = 2.5e6 \\
        $k_p$ & gradually increase from 1 to 8 \\
        $k_q$ & 4 \\
        \midrule
        %$\lambda_0$ & 1 \\
        $\lambda_1$ & 0.001 \\
        $\lambda_2$ & 0.1 \\
        $\lambda_3$ & 0.01 \\
        \bottomrule
    \end{tabular}
    \label{tbl_hyper}
\end{table}



\section{Related Work}

%\cite{vondrick2016generating}
%\cite{byravan2017se3}
%\cite{choi2018contingency}

The problem of action conditioned frame prediction in Atari games has been studied in \cite{DBLP:conf/nips/OhGLLS15} and \cite{DBLP:journals/corr/LeibfriedKH16}. They both adopt a three stage neural network based Encoding-Transformation-Decoding framework for predicting the future frame from the action and previous frames. In the transformation stage, the element-wise product between the encoded frame representation vector and the action embedding is computed as the representation of the future frame. However, the controllable image regions are not explicitly isolated in these works. Neither do they investigate the possibility of using the predicted images as input to an RL agent to boost performance. Similar action-conditioned future frame prediction has also been studied in robotic vision\cite{DBLP:conf/nips/FinnGL16, DBLP:conf/icra/FinnL17}, while following the similar framework but adopting a more complex neural network architecture including cross convolutions and attention masks. As for the real world future video prediction, \cite{vondrick2016generating} adopts a foreground background separation framework similar to us, but their method is not directly applicable to action conditioned prediction. There are also prediction methods operating on other kinds of sensory input, such as point cloud \cite{byravan2017se3}.

\cite{DBLP:conf/aaai/BellemareVB12} studies the problem of learning contingent regions, which is formalized as the parts of observation whose immediate future pixel value depends on the agent's action, from Atari game replays. The definition of contingent regions resembles our mask for controllable objects. However, we propose a deep learning based framework for the more effective learning of such regions, instead of traditional pixel-level transition models in \cite{DBLP:conf/aaai/BellemareVB12}.

The idea of using prediction error as exploration bonus or intrinsic motivation for RL has been seen in \cite{DBLP:conf/icml/PathakAED17, DBLP:journals/corr/StadieLA15}. \cite{DBLP:conf/nips/BellemareSOSSM16} further relates prediction error as intrinsic motivation to count-based exploration by deriving a pseudo count from an arbitrary density model. In this paper, we draw on this idea and demonstrate that the prediction error in our model can also be used as exploration bonus. An concurrent work \cite{choi2018contingency} studies contingency awareness which is also defined as the controllable part of observation to promote better exploration for A2C algorithm. But they only use the contingency region as representation for count-based exploration method, and did not investigate the use of contingency region as input or prediction error as bonus. In this paper, we demonstrate that using contingency region directly as additional input already provides useful signal for the agent to facilitate learning, and simply adding the prediction error as bonus is also effective.

Finally, the video prediction model can also used as models of the environment dynamics in model-based RL learning, e.g. \cite{DBLP:journals/corr/WeberRRBGRBVHLP17, hafner2018learning, kaiser2019model}, where the predicted future state roll-outs are used as the imagination of the agent. These methods are often sensitive to the accuracy of the learned dynamics at longer time scale as the error may accumulate with more prediction time steps, while our method only require one-step prediction to be reasonably well. Dense image prediction can also be employed as an auxiliary task to train the agent's CNN better \cite{DBLP:journals/corr/JaderbergMCSLSK16}. However, the focus of this paper is to introduce a framework to learn the separation of controllable object, and to study whether such separation can benefit \emph{model-free} RL training, rather than to exploit every possible use of prediction model.


